Interpreting Verbal Irony: Linguistic Strategies and the Connection to the Type of Semantic Incongruity

Human communication often involves the use of verbal irony or sarcasm, where the speakers usually mean the opposite of what they say. To better understand how verbal irony is expressed by the speaker and interpreted by the hearer we conduct a crowdsourcing task: given an utterance expressing verbal irony, users are asked to verbalize their interpretation of the speaker's ironic message. We propose a typology of linguistic strategies for verbal irony interpretation and link it to various theoretical linguistic frameworks. We design computational models to capture these strategies and present empirical studies aimed to answer three questions: (1) what is the distribution of linguistic strategies used by hearers to interpret ironic messages?; (2) do hearers adopt similar strategies for interpreting the speaker's ironic intent?; and (3) does the type of semantic incongruity in the ironic message (explicit vs. implicit) influence the choice of interpretation strategies by the hearers?

==> charac_strategies_evaluation.tex <==
\section{Irony Properties and Rephrasing Strategies} \label{section:propstrategies} 

Table \ref{table:propstrategies} represents the correlation of Turkers' rephrasing strategies over S$_{im}$-H$_{int}$ corpus against the type of the incongruence. $Exp.$ & $Imp.$ respectively show the cases for explicit and implicit incongruence.

\begin{table}[h]
\centering
\begin{small}
\begin{tabular}{p{3 cm}p{.6cm}p{.6cm}p{.6cm}p{.6cm}}
%p{.6cm}p{.6cm}p{.6cm}p{.6cm}p{.6cm}}
\hline
Strategies & \multicolumn{2}{c} {$incongruence$} & \multicolumn{2}{c} {$marker$}  \\
& $Exp.$ & $Imp.$ & $P$ & $A$ \\
%Strategies & \multicolumn{3}{|c|} {a} & \multicolumn{3}{c|}  {b}\\
\hline
Lex\_ant  &  \emph{48.5} & 34.8 & 35.7 & \emph{42.2} \\
Simple\_neg & 24.9 & 32.3 & 28.9 & 30.0 \\
AN\_weaksent &  14.3 &  17.6 & 15.7 & 16.8 \\
AN$_{I \rightarrow D}$  & 5.9 &  6.1 & 12.3  & 3.1 \\
AN\_desiderative & 1.3 & 1.90 & 0.9 & 2.0 \\
AntPhrase+PragInf & 5.2 & 7.1 & 6.2 & 6.6 \\
\hline
\end{tabular}
\caption{Rephrasing Strategies against Incongruency and Irony Markers (in \%)}
\label{table:propstrategies}
\end{small}
\end{table}

We observe when incongruence is present explicitly in the utterances Turkers rephrase it with lexical antonyms more than when it is implicit (48.5\% vs. 34.8\%). As stated earlier in section \ref{section:charac}, majority of the explicit incongruence appears when an utterance contains sentiment words of opposite polarity. Thus, we find Turkers' rephrase such examples with direct lexical antonyms. 

We also analyze the rephrasing strategies in the light of occurrence of irony markers ($P$ and $A$ columns denote the presence and absence of markers, respectively).  Recall, irony markers are indicators of irony that assists the recognition of the phenomena. We implement various morpho-syntactic as well as typographic markers (similar to \cite{ghosh20181}) to identify the presence of markers. We observe $Lex\_ant$ strategy is most used in cases where the markers are absent. With a thorough analysis of the S$_{im}$-H$_{int}$ corpus we found markers are used more than twice in case of implicit incongruence vs. explicit ones (i.e., 21\% vs. 10\%, respectively). In many such cases (e.g., ``I have always loved studying ;) '', ``packing is so much fun !!!'') the inconruency is hidden within the \textit{context} that is absent in the utterances. However, in such cases, Turkers mostly changed the sentiment word (e.g., ``love'' $\leftrightarrow$ ``hate''; fun $\leftrightarrow$ ``boring'') to its opposite.  


==> strategies_acl2019.tex <==
\section{Interpreting Verbal Irony: A Typology of Linguistic Strategies} \label{section:strategies}
\subsection{Interpreting Verbal Irony}
%Cross Linguistic Typology of Strategies Indicating irony} \label{section:strategies}
%SM should we replace Irony by "sarcasm" ? Examples were collected using "sarcasm" hashtags.... 


%Why we have experimented with the SM data and used the Turkers to generate the rephrases? First of all, as SMs have the opposite valence (i.e., the intended meaning is usually the opposite of the literal) the Turkers are easily able to generate IMs and the SM-IM data can be treated as a contradiction dataset and IM-IM data as the paraphrase dataset (See Table \ref{table:sarcs} for examples). Second, we can conduct different types of alignments over the SM-IM and IM-IM data to extract paraphrases and antonym phrases since a) different Turkers may paraphrase differently to replace the sarcastic meaning and b) use antonyms to show the intended meaning is opposite of the literal. 

%cross-linguistic strategies/language specific strategies/ mapping with theoretical framework : across-languages/language specific and pragmatic inferences in the specific--- then: impact for the theoretical frameworks 


%In this section, we propose a typology of linguistic strategies used in hearers' interpretations of speakers' ironic messages. 
%SM we should put this in data, saying we focus on verbal irony where some notion of opposite meaning 
Given the definition of verbal irony, we would expect that Turkers' interpretation of speaker's ironic message will contain some degree of opposite meaning w.r.t. to what the speaker's said. However, it is unclear what linguistic strategies the Turkers will use to express that. 
%SM I put this in intro and I'll bring it back in related work
%Our methodological assumption is that since irony is an interactional phenomenon with specific perlocutionary effects \cite{haverkate1990speech}, the analysis of how ironical utterances are perceived and interpreted by potential hearers is crucial to identify linguistic strategies expressing irony. 
%SM for Spanish I put 3950 since only 50 were rejected and we had 800 tweets.
To build our typology, from the total set of S$_{im}$-H$_{int}$ pairs obtained through crowdsourcing (i.e., 4,762 pairs; see Section \ref{section:data}) we selected a $dev$ set of 500 S$_{im}$-H$_{int}$ pairs. % to manually compare and contrast each pair of utterances containing speaker's sarcastic message and hearer's interpretation. 
 A linguist expert in semantics and pragmatics analyzed the $dev$ set proposed the typology of linguistic strategies, thus our approach is bottom-up, data-driven.  The core linguistic strategies are explained below and synthesized in Table \ref{table:distrigold}.

%In addition, these strategies provide a testbed for the explanatory potential of theoretical frameworks of irony.
%
%Their distribution depends on linguistic features of the ironic utterance; they provide a testbed for the explanatory potential of linguistic theoretical frameworks. 
%DG:In the following subsection we briefly discuss the identified linguistic strategies, and then link these strategies to theoretical framework of interpreting verbal irony.
%EM I think we can deleter this last paragraph since redundant 
% starting from 

%DG: Shortening.
\subsection{Linguistic Strategies}
\paragraph{Lexical and phrasal antonyms:}This category contains the lexical antonyms (e.g., ``love''  $\leftrightarrow$ ``hate'', ``great'' $\leftrightarrow$ ``terrible'') as well as indirect antonyms \cite{fellbaum1998wordnet}, where the opposite meaning can only be interpreted in context (e.g., ``{passionate} speaker'' $\rightarrow$ ``{boring} speaker''; Table \ref{table:sarcesboth}). Although the typical antonym of  ``passionate'' is ``unpassionate'', ``boring'' works in this context as a lexical \emph{opposite} since a speaker who is passionate entails that he is not boring. 
%DG:commented since we have the table. Lexical antonyms were used as strategy in 38\% of cases in English and 52\% in Spanish (Table \ref{table:distrigold}).
%This type of antonyms is usually referred to in the linguistic literature as \emph{indirect} antonyms \cite{fellbaum1998wordnet}. 
%\paragraph{Lexical and phrasal Antonyms (English/Spanish):}This category refers to lexical opposites that we are labeling as \emph{direct} antonyms ( e.g., English ``love''  $\leftrightarrow$ ``hate'', ``great'' $\leftrightarrow$ ``terrible''; Spanish ``amo''  $\leftrightarrow$ ``odio'',  ``madurez'' $\leftrightarrow$ ``inmadurez'', ``madurez'' $\leftrightarrow$ ``inmadurez''). We consider antonyms also those words which, despite not being the direct antonym of the corresponding term in the ironic sentence, bear an opposite meaning in the context of utterance, i.e., ``ed davey is such a \emph{passionate}, inspiring speaker'' $\rightarrow$``ed davey is such a \emph{boring}, inspiring speaker'', working as lexical opposite. Although typical antonyms of  ``passionate'' are ``unpassionate'' and ``uncaring'', ``boring'' works in this context as a lexical \emph{opposite} since the fact that a speaker is passionate entails that he is not boring.This type of antonyms is usually referred to in the linguistic literature as \emph{indirect} antonyms \cite{fellbaum1998wordnet}. 
Besides lexical antonyms, Turkers sometimes use
%EM use 
antonym phrases (e.g., ``I can't wait'' $\rightarrow$ ``not looking forward'', ``I like (to visit ER)'' $\rightarrow$ ``I am upset (to visit ER) '').% Antonym phrases were used in 5\% of cases in English and 7\% in Spanish.  %However, the lexical choices used to build the phrases are difficult to predict. 

%DG: what about beliefs? 
%The strategy of antonyms (direct/indirect/phrases) is used by Turkers mainly when the trigger of irony in the ironic utterance is a word/phrase expressing sentiment.

\paragraph{Negation:} Here, Turkers negate the main predicate. This strategy is used in the presence of copulative constructions where the predicative expression is an adjective/noun expressing sentiment (e.g., ``is great'' $\rightarrow$ ``is \textbf{not} great'') and of verbs expressing sentiment (e.g., ``love'' $\rightarrow$ ``\textbf{do not} love'') or propositional attitudes (e.g., ``I wonder'' $\rightarrow$ ``I \textbf{don't} wonder''). 
\begin{table}
\begin{center}
\begin{small}
\begin{tabular}{lc}
\hline
Typology & Distribution (\%)\\
\hline
\textbf{Antonyms} & \\
 - lexical antonyms &  (42.2) \\
 - antonym phrases &  (6.0)\\
\textbf{Negation} & \\
 - simple negation &  (28.4) \\
\textbf{Antonyms OR Negation} & \\
 - weakening sentiment &  (23.2)\\
 - interrogative $\rightarrow$ declarative  &  (5.2)\\
 - desiderative constructions &  (2.8)\\
\textbf{Pragmatic inference}&  (3.2)\\
\hline
\end{tabular}
\end{small}
\end{center}
\caption{Typology of linguistic strategies and their distribution (in \%) over the $dev$ set}
\label{table:distrigold}
\end{table}
\paragraph{Weakening the intensity of sentiment:} The use of negation and antonyms is sometimes 
%EM maybe rephrase: the use of negation and antonysms is sometimes 
accompanied by two strategies that reflect a weakening of sentiment intensity. First, when S$_{im}$ contains words expressing a high degree of positive sentiment, the hearer's interpretation replaces them with more neutral ones (e.g., ``I \textbf{love} it'' $\rightarrow$ ``I don't \textbf{like} it''). Second, when S$_{im}$ contains an intensifier, it is eliminated in the Turkers' interpretation. Intensifiers  specify the degree of the value/quality expressed by the words they modify \cite{mendez2008special} (e.g., ``cake for breakfast. \textbf{so} healthy'' $\rightarrow$ ``cake for breakfast. \textbf{not} healthy''). 
%SM what is the intensifier in the above example for spanish? 
%These strategies accounted for 21\% of cases in English and  8\% in Spanish. 
 
%SM The above lindaaas is more like an intensifier since it is the elongation of the words aaaas like coool in english. No ? Also in the above example for spanish is replaced with an antonym... sO maybe not a parallel with love -> don't like. 
%add Spanish claro ques

%``I just really enjoy getting fucked over''$\rightarrow$ ``I hate getting fucked over''; ``estudios sociales es tan bonito''$\rightarrow$ ``Estudios sociales es aburrido''

% SM burgers2012verbal was given an error so I took it out 
%SM I commented this since the logic to me is not correct: we are not talking about removign the marker and then trying to perceive sarcasm, so I am not sure what this sentence tries to get at. And we need to save space
%Intensifiers as well as words expressing a high degree of sentiment express the trope of hyperbole. Therefore, it seems that this figure of speech is perceived as an \emph{irony marker} \cite{attardo2000ironyb}, a meta-communicative clue which instructs hearers in the interpretation process: if the linguistic items expressing hyperbole are removed, the sentence is still ironic, but less easy to interpret. 

% SM I am changing this to remove confusing 
\paragraph{Interrogative to Declarative Transformation (+ Antonym/Negation).} This strategy, used mostly in conjunction with the negation or antonym strategies is to replace the interrogative form with a declarative form, when S$_{im}$ is a rhetorical question (for brevity, $RQ$) (e.g., ``don't you \textbf{love} fighting?'' $\rightarrow$ ``I \textbf{hate} fighting''). %$RQ$s are deemed as a pragmatic strategy \cite{muecke1969compass} to be accounted for regarding pretense and indirect assertion \cite{kaufer1981understanding,recanati2004literal,frank1990you}. %: the speaker does not mean to ask a question but simply pretends to perform one.% These strategy accounted for 5\% of cases in English and 1\% in Spanish. 

%SM I am not entirely sure what is here... So these are not rhetorical questions, why are they here? And we need to save space, so I am commenting them out
% In some cases, question marks in the sarcastic meaning do not signal the presence of a question but bear the same function of exclamation marks, working as the intensifiers at the illocutionary level (i.e. ``i sprayed perfume in my eye! i am now a genius!!?''$\rightarrow$``i sprayed perfume in my eye, what a dumb thing to do!'')
 
%; ``sida ?. embarazo ?. mala vida en el futuro ?. donde ?'' $\rightarrow$ ``la noticia del embarazo es buena''). 
%used when the hearer's interpretation is the semantically opposite of what the speaker said 

\paragraph{Counterfactual Desiderative Constructions:} When the ironic utterance expresses a positive/negative sentiment towards a past event (e.g., ``glad you relayed this news'') or an expressive speech act (e.g., ``thanks $X$ that picture needed more copy'') the hearer's interpretation of intended meaning is expressed through the counterfactual desiderative constructions \textit{I wish (that) p} (``\textbf{I wish} you hadn't relayed \dots'', ``\textbf{I wish} $X$ didn't copy \dots'').
%This strategy is distinguished from the antonymic phrases since it stresses on the failure of the speaker's expectation more than on his commitment to the opposite meaning.
Differently from antonymic phrases, this strategy stresses on the failure of the speaker's expectation more than on their commitment to the opposite meaning.

\paragraph{Pragmatic Inference:} In addition to the above strategies, there are cases where the interpretation calls for an inferential process to be recognized. For instance, ``made 174 this month \dots \textit{I'm gonna buy a yacht!}'' $\rightarrow$ ``made 174 this month \dots \textbf{I am so poor}". % Pragmatic inference strategy was applied in 3\% of cases in English and 5\% in Spanish. 
%DG removing the following line:
% The above strategies were found in both English and Spanish. In our development set we identified only two strategies that are specific to either English or Spanish:
%
The distribution of the strategies on the $dev$ set is represented in Table \ref{table:distrigold}.
%This strategy accounted for more than 2\% of cases in English. 
%add that it can also be the case with expressive speech acts  

%\paragraph{Epistemic certitude (Spanish):}  
%EM delete in Spanish: redundant 
%Adverbs indicating epistemic certitude having sentential scope are used besides intensifiers as sarcasm indicators. In H$_{int}$, Turkers drop these markers to weaken the epistemic commitment to the truth of the proposition, showing that they perceive their sarcastic function (e.g., ``\textbf{claro} es buensiima xq se lo pasoo" $\rightarrow$ ``es malo que se lo paso"). % This strategy accounted for 1.2\% of cases in Spanish. 
%\subsection{}

 \subsection{Links to Theoretical Frameworks} \label{section:theory}
 
In the linguistic literature many different approaches to irony have been provided. According to  \citet{grice1975syntax}, ironic messages are uttered to convey a meaning opposite to that literally expressed, flouting the conversational maxim of Quality ``do not say what you believe to be false''. In verbal irony, the violation of the maxim is frequently signaled by ``the opposite'' of what is said literally (e.g., intended meaning of ``carcasses are flattering'' is they are gross; Table \ref{table:sarcesboth}).  
the linguistic strategies of \textit{antonyms} (e.g. ``worst day of my life") and simple \textit{negation} (``yeap we totally dont drink alcohol every single day''[...]) cover majority of the S$_{im}$-H$_{int}$ corpus and can be explained by the Gricean \cite{grice1975syntax} account of irony, since the hearer seems to have primarily recognized the presence of semantic incongruity. 
%EM_july
In contrary, as touched upon by \newcite{giora1995irony}, \textit{antonyms} and \textit{direct negation} are not always semantically equivalent strategies, since the second sometimes allows a graded interpretation: if ``x is not encouraging", it is not necessarily bad, but simply ``x $<$ encouraging''. Such an implicature is available exclusively with items allowing mediated contraries, such as sentiment words \cite{horn1989natural}. Direct negation with sentiment words implies that just one value in a set is negated, while the others are potentially affirmed.
%the scope of the set of possible values is larger with words that express a strong sentiment than with words that express a weak one.  
%EM July 
The spectrum of interpretations allowed by negation as a rephrasing strategy indicates that hearers recognize that the \emph{relevance} of the ironic utterance in itself plays a role next to what the utterances refers to (if the rephrased utterance is intended as ``x is not encouraging at all'', the perceived irrelevance of the corresponding ironic  utterance is more prominent than in ``x is not very encouraging"). 
The fact that the interpretation of irony has a propositional scope is even more clear when the ironic sentence in interrogative form (``And they all lived happily ever after ?") is rephrased as a declarative (e.g. ``I doubt they all lived happily ever after"): the hearers recognizes that the question has a rhetoric value since contextually irrelevant otherwise. The intentional falsehood of Gricean analysis is also not deemed by \citet{wilson2012explaining} as a necessary and sufficient condition for irony. According to their theory of \emph{echoic mentioning}, irony presupposes the mention to the inappropriateness of the entire sentence: in asserting ``Awesome weather in Scotland today" the speaker does not simply want to express that the weather was horrible but he signals that assuming that the weather would be nice was irrelevant and, thus, ridiculous. \citet{kreuz1989sarcastic} expand the Relevance Theory approach talking about \emph{echoic reminding} to account for cases such as ``Could you be just a little louder, please? My baby isn't trying to sleep" where the extreme politeness reminds the hearer that the question is indeed a request and that the mother bears a certain stance and has certain expectations towards the addressee.
Similarly, the use of the \emph{pragmatic strategy} cannot be fully explained in Gricean terms: the rephrase ``made 174 this month \dots I am so poor'' for ``made 174 this month \dots I am gonna buy a yatch'' more than pointing to the presence of lexical incongruity, show that the hearers knows for background knowledge that the assertion of ``buying a yatch'' is completely irrelevant in the context of a low salary situation. 
Rephrasing strategies using counterfactual desiderative constructions (e.g. ``I really wish my friends and family would check up on my after yesterday's near death experience") show, instead, that the interpretation of irony involves an \emph{echoic reminding} to the speaker's (social) expectations which failed to be fulfilled.
%EM_july: not sure weather the following is useful or not
Overall, using the results of our crowdsourcing experiment with main existing theories of irony, it turns out that the theories have a complimentary explanatory power. In (Section \ref{section:tweets}) we investigate weather this situation might relate to the presence of explicit/implicit irony (cfr. section 6). 
 
 
 
 


